Towards machine learning guided by best practices

Nowadays, machine learning (ML) is being used in software systems with multiple application fields, from medicine to software engineering (SE). On the one hand, the popularity of ML in the industry can be seen in the statistics showing its growth and adoption. On the other hand, its popularity can also be seen in research, particularly in SE, where not only have multiple studies been published in SE conferences and journals but also in the multiple workshops and co-located conferences in software engineering conferences. At the same time, researchers and practitioners have shown that machine learning has some particular challenges and pitfalls. In particular, research has shown that ML-enabled systems have a different development process than traditional SE, which also describes some of the challenges of ML applications. In order to mitigate some of the identified challenges and pitfalls, white and gray literature has proposed a set of recommendations based on their own experiences and focused on their domain (e.g., biomechanics), but for the best of our knowledge, there is no guideline focused on the SE community. This thesis aims to reduce this gap by answering research questions that help to understand the practices used and discussed by practitioners and researchers in the SE community by analyzing possible sources of practices such as question and answer communities and also previous research studies to present a set of practices with an SE perspective.

==> secs/approach.tex <==
% !TEX root = main.tex

\section{Content}

Add all your missing sections here \\


\input{tables/dfltTable}



All resources must be referenced using \lstinline[basicstyle=\small\ttfamily]|\fref{}|

\fref{lst:test}
\fref{fig:test}
\fref{tab:test}

\begin{lstlisting}[caption={test},label={lst:test}]
Test
\end{lstlisting}

In case the author needs to present a folder structure \textcolor{red}{dirtree} package can be used:



==> secs/conclusion.tex <==
% !TEX root = main.tex

\section{Conclusion \& Future Work}


==> secs/content.tex <==
% !TEX root = main.tex

\section{Content}

Add all your missing sections here \\


\input{tables/dfltTable}

\begin{figure}[!h]
\centerline{\includegraphics[width=0.8\linewidth]{imgs/logoSquare.png}}
\caption{Example of a figure caption.}
\label{fig:test}
\end{figure}

All resources must be referenced using \lstinline[basicstyle=\small\ttfamily]|\fref{}|

\fref{lst:test}
\fref{fig:test}
\fref{tab:test}

\begin{lstlisting}[caption={test},label={lst:test}]
Test
\end{lstlisting}

In case the author needs to present a folder structure \textcolor{red}{dirtree} package can be used:

\begin{figure}[h]
	\centering
	\fbox{%
		\parbox{\dimexpr\linewidth-6\fboxsep-6\fboxrule}{%
			\fontsize{8pt}{8pt}
			\begin{minipage}[t]{\linewidth}
				\dirtree{%
					.1 /.
					.2 bin.
					.2 home.
					.3 jeancome.
					.4 texmf.
					.5 tex.
					.3 jeancomeson\DTcomment{Guillaume}.
					.3 jeancomedaughter\DTcomment{Mathilde}.
					.2 usr.
					.3 bin.
				}
			\end{minipage}\hfill
		}
	}
	\caption{Example Directory Tree}
	\label{fig:dirtree}
\end{figure}%



==> secs/introduction.tex <==
% !TEX root = main.tex

\section{Introduction}



However, recent papers have discussed different challenges, limitations and pitfalls of using Machine Learning without following the appropriate guidelines and best practices. 







==> secs/study.tex <==
% !TEX root = main.tex

\section{Conclusion \& Future Work}


==> tables/dfltTable.tex <==
\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab:test}
\end{center}
\end{table}
